UV Spectra, Line Indices of M31 Globular Clusters and E Galaxy Cores

Observations in integrated light (2200-4800 A, 8 to 11 A resolution, S/N > 20) of 4 M31 globular clusters and of the cores of six gE galaxies made with the HST/FOS are presented and analyzed. These data are supplemented by IUE observations of M32, Galactic globulars and stars. From these data we measure UV colors and absorption line strength (ALS) indices, including the key NH feature at 3360 A. We find that our data divide the M31 globular clusters, Galactic globular clusters/Galactic stars, and gE galaxies into three different stellar populations. The old stellar populations of M31 globular clusters and elliptical galaxies are more similar to each other than each is to the Galactic stellar population. Of special note is that the NH feature is so strong in the spectra of M31 globulars that a large (>20) overabundance in nitrogen in these stars, relative to that in Galactic stars, is likely required. Other ALS indices (of Mg, Al) also show significant differences.

==> ponder.tab1_2.tex <==
\begin{planotable}{lllccccccccrl}
\tablewidth{0pt}
\tablecaption{FOS Observational Parameters: M31 Globular Clusters and 
Elliptical Galaxies}
\tablenum{1}
\tablehead{
\multicolumn{1}{c}{Name}                & \multicolumn{1}{c}{R. A.} &
\multicolumn{1}{c}{Dec}         & \multicolumn{1}{c}{E(B--V)} &
\multicolumn{1}{c}{Mg$_2$} &    \multicolumn{1}{c}{V$\rm _H$} &
\multicolumn{1}{c}{Data Set}            & \multicolumn{1}{c}{Date of } &
\multicolumn{2}{c}{Obs Times (sec)}	& \multicolumn{1}{c}{Other}
\\
\multicolumn{1}{c}{}                    & \multicolumn{2}{c}{(J2000)} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &  \multicolumn{1}{c}{km s$^{-1}$} &
\multicolumn{1}{c}{ID$^{1}$}            & \multicolumn{1}{c}{Obs}&
\multicolumn{1}{c}{Exposure}	        & \multicolumn{1}{c}{Setup} &
%\multicolumn{1}{c}{Total Time}		& 
\multicolumn{1}{c}{Names$^{2}$}}
\startdata
Globular Clusters &&&&&&&&&& \nl
\hline \nl
K58  &00:40:26&+41:27:26&0.080&0.213&-213&y17c01$\ldots$ & 21/01/93 &2756&1485& V55, Bol 6 \nl
K280 &00:44:29&+41:21:35&0.080&0.184&-164&y17c04$\ldots$ & 17/10/93 &2794&705& V282, Bol 225 \nl
MII  &00:32:46&+39:34:39&0.080&0.148&-331& y17c52$\ldots$ & 19/11/93&2794&450& K1 \nl
     &        &         &&& & y17c0206t & 18/01/93 &0$^{3}$&0&   \nl
MIV  &00:43:17&+39:49:12&0.080&0.038&-270&y17c03$\ldots$ & 20/01/93&2794&825& K219, Bol 358 \nl
\hline \nl
Ellipitical Galaxies &&&&&&&&&& \nl
\hline \nl
NGC 3605&11:16:46&+18:01:02&0.000&0.241&649&y39x01$\ldots$ & 06/06/96 &10600&1408& UGC 6295\nl
NGC 3608&11:16:58&+18:08:55&0.000&0.329&1205&y39x02$\ldots$ & 06/12/96 &10600&958& UGC 6299\nl
NGC 5018&13:13:01&-19:31:07&0.055&0.210&2794&y39x03$\ldots$ & 20/12/96 &10600&1408& UGCA 335\nl
NGC 5831&15:04:07&+01:13:10&0.040&0.303&1924&y39x06$\ldots$ & 28/07/96 &10600&1102& UGC 9678\nl
NGC 6127&16:19:11&+57:59:03&0.035&0.322&4609&y39x04$\ldots$ & 13/07/96 &9030&1453& NGC 6128, UGC 10345 \nl
NGC 7619&23:20:14&+08:12:21&0.000&0.358&3804&y39x05$\ldots$ & 13/07/96 &3370&1408& UGC 12523   \nl
        &        &         & &&& y39x55$\ldots$ & 22/11/96&10600&1408& \nl
\tablenotetext{1}{The data identification is in the form of instrument name
(y=FOS), program ID (39x or17c), and observation set ID (eg. 55).  The last
three fields (replaced with $\ldots$) are individual exposures within that set
of observations.}
\tablenotetext{2}{Names taken from SIMBAD.  K = Sargent et al. 1977 numbers; 
Bol = Bologna numbers, taken from Battistini et al. 1980; 1987.}
\tablenotetext{3}{observed with G130H grating on Blue detector --- 
unusable due to geo-coronal L-alpha and OI 1300 emission}
\end{planotable}

\begin{planotable}{lrrrrrrrrl}
\tablewidth{0pt}
\tablecaption{Definitions for Line Indices and Colors}
\tablenum{2}
\tablehead{
\multicolumn{1}{c}{Feature Name}	& \multicolumn{2}{c}{Blue Passband} &
\multicolumn{4}{c}{Index Passband}	& \multicolumn{2}{c}{Red Passband} &
\multicolumn{1}{c}{Comments \& Source}
\\
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{($\rm \AA$)} &
\multicolumn{1}{c}{($\rm \AA$)} &
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{($\rm \AA$)} &
\multicolumn{1}{c}{($\rm \AA$)} &
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{($\rm \AA$)} &
\multicolumn{1}{c}{($\rm \AA$)} &
}

\startdata
\hline \nl
2600--3000   & 2470 & 2670 &\hspace*{5mm}&\nodata&\nodata&\hspace*{5mm}& 2930 & 3130 & 3, FOBW (1990) \nl
Fe II 2402   & 2285 & 2325 &\hspace*{5mm}& 2382 & 2422 &\hspace*{5mm}& 2432 & 2458 &  2,    "  \nl
BL 2538      & 2432 & 2458 &\hspace*{5mm}& 2520 & 2556 &\hspace*{5mm}& 2562 & 2588 &  2,    " \nl
Mg Wide      & 2470 & 2670 &\hspace*{5mm}& 2670 & 2870 &\hspace*{5mm}& 2930 & 3130 &  2,    " \nl
Fe II 2609   & 2562 & 2588 &\hspace*{5mm}& 2596 & 2622 &\hspace*{5mm}& 2647 & 2673 &  2,    " \nl
2609/2660    & 2596 & 2623 &\hspace*{5mm}&\nodata&\nodata&\hspace*{5mm}& 2647 & 2673 &  3,    " \nl
Fe I+II + CrI& 2647 & 2673 &\hspace*{5mm}& 2736 & 2762 &\hspace*{5mm}& 2762 & 2782 &  2,    " \nl
Mg II 2800   & 2762 & 2782 &\hspace*{5mm}& 2784 & 2814 &\hspace*{5mm}& 2818 & 2838 &  2,    " \nl
Mg I 2852    & 2818 & 2838 &\hspace*{5mm}& 2839 & 2865 &\hspace*{5mm}& 2906 & 2936 &  2,    " \nl
2828/2921    & 2818 & 2838 &\hspace*{5mm}&\nodata&\nodata&\hspace*{5mm}& 2906 & 2936 &  3,    " \nl
Fe I 3000    & 2906 & 2936 &\hspace*{5mm}& 2965 & 3025 &\hspace*{5mm}& 3031 & 3051 &  2,    " \nl
BL 3096      & 3031 & 3051 &\hspace*{5mm}& 3086 & 3106 &\hspace*{5mm}& 3115 & 3155 &  2,    " \nl 
UV continuum & 3150 & 3250 &\hspace*{5mm}&\nodata&\nodata&\hspace*{5mm}& 4180 & 4290 &  3, Davidge\&Clark (1994) \nl
NH 3360      & 3320 & 3350 &\hspace*{5mm}& 3350 & 3400 &\hspace*{5mm}& 3415 & 3435 &  1,    " \nl
Bl 3580      & 3500 & 3540 &\hspace*{5mm}& 3540 & 3600 &\hspace*{5mm}& 3620 & 3650 &  1,    " \nl
Balmer       & 3600 & 3700 &\hspace*{5mm}&\nodata&\nodata&\hspace*{5mm}& 4250 & 4290 &  3,    " \nl
4000         & 3750 & 3950 &\hspace*{5mm}&\nodata&\nodata&\hspace*{5mm}& 4050 & 4250 &  3,    " \nl
CN 3883      & 3760 & 3780 &\hspace*{5mm}& 3780 & 3900 &\hspace*{5mm}& 3900 & 3915 &  2,    " \nl
Ca HK        & 3900 & 3915 &\hspace*{5mm}& 3915 & 4000 &\hspace*{5mm}& 4000 & 4020 &  1,    " \nl
CN 4170      & 4082 & 4118 &\hspace*{5mm}& 4144 & 4178 &\hspace*{5mm}& 4246 & 4284 &  2, BFGK (1984) \nl
CH = G 4300  & 4268 & 4283 &\hspace*{5mm}& 4283 & 4317 &\hspace*{5mm}& 4321 & 4336 &  1,    " \nl
Fe 4383      & 4360 & 4372 &\hspace*{5mm}& 4370 & 4422 &\hspace*{5mm}& 4444 & 4456 &  1, Worthey {\em et al.} (1994)  \nl
Ca 4455      & 4447 & 4455 &\hspace*{5mm}& 4453 & 4476 &\hspace*{5mm}& 4478 & 4493 &  1,    "\nl
Fe 4531      & 4506 & 4516 &\hspace*{5mm}& 4516 & 4561 &\hspace*{5mm}& 4562 & 4581 &  1,    "\nl
C$_{2}$ 4668 & 4613 & 4632 &\hspace*{5mm}& 4635 & 4722 &\hspace*{5mm}& 4744 & 4758 &  1,    "\nl
\tablenotetext{1}{1 = Equivalent width (in $\rm \AA$); 2 = magnitude; 
3 = band ratio or color (in mag)}
\end{planotable}



==> ponder.tab3.tex <==
\begin{planotable}{lcrrrrrrrrrr}
\tablewidth{0pt}
\tablecaption{Ultraviolet/Violet Spectral Indices and Colors - Globular Clusters}
\tablenum{3a}
\tablehead{
\multicolumn{1}{c}{Feature}             & \multicolumn{1}{c}{Type$^1$} &
\multicolumn{2}{c}{M32} &
\multicolumn{2}{c}{K58}                 & \multicolumn{2}{c}{K280} &
\multicolumn{2}{c}{MII}                 & \multicolumn{2}{c}{MIV}
\\ 
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err$^2$} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} 
}
\startdata
\hline\nl
 2600--3000&3&   1.496 & \nodata &   1.509& 0.047 &   1.003& 0.013 &   0.689& 0.008 &   0.373& 0.014\nl
Fe II 2402 &2& \nodata & \nodata &   1.453& 0.554 &   0.182& 0.066 &   0.287& 0.039 &   0.244& 0.064\nl
   BL 2538 &2&   0.483 & \nodata &   0.735& 0.302 &   0.331& 0.063 &   0.348& 0.038 &   0.212& 0.060\nl
   Mg Wide &2&   0.264 & \nodata &   0.228& 0.037 &   0.200& 0.012 &   0.097& 0.009 &   0.018& 0.015\nl
Fe II 2609 &2&   0.458 & \nodata &   0.616& 0.162 &   0.383& 0.044 &   0.407& 0.027 &   0.219& 0.046\nl
 2609/2660 &3&   0.799 & \nodata &   0.990& 0.143 &   0.633& 0.038 &   0.578& 0.025 &   0.265& 0.041\nl
Fe I+II +C &2&   0.357 & \nodata &   0.444& 0.142 &   0.247& 0.046 &   0.188& 0.031 &   0.074& 0.050\nl
Mg II 2800 &2&   0.737 & \nodata &   1.127& 0.160 &   0.693& 0.044 &   0.650& 0.028 &   0.368& 0.046\nl
 Mg I 2852 &2&   0.358 & \nodata &   0.583& 0.105 &   0.401& 0.035 &   0.320& 0.024 &   0.069& 0.040\nl
 2828/2921 &3&   0.534 & \nodata &   0.608& 0.085 &   0.490& 0.030 &   0.327& 0.021 &   0.061& 0.037\nl
 Fe I 3000 &2&   0.177 & \nodata &   0.195& 0.061 &   0.156& 0.024 &   0.122& 0.018 &   0.012& 0.033\nl
   BL 3096 &2&   0.100 & \nodata &   0.252& 0.072 &   0.206& 0.028 &   0.146& 0.022 &   0.063& 0.041\nl
UV continuum &3& \nodata & \nodata &   1.141& 0.025 &   1.126& 0.009 &   0.877& 0.008 &   0.680& 0.016\nl
   NH 3360 &1& \nodata & \nodata &   7.879& 2.973 &   8.253& 1.062 &   7.560& 0.912 &   3.687& 2.052\nl
   Bl 3580 &1& \nodata & \nodata &   7.241& 2.615 &   8.965& 0.962 &   4.366& 0.880 &  -0.429& 1.960\nl
    Balmer &3& \nodata & \nodata &   0.684& 0.031 &   0.637& 0.012 &   0.580& 0.010 &   0.495& 0.023\nl
      4000 &3& \nodata & \nodata &   0.616& 0.018 &   0.643& 0.007 &   0.456& 0.006 &   0.202& 0.012\nl
   CN 3883 &2& \nodata & \nodata &   0.286& 0.055 &   0.333& 0.020 &   0.200& 0.017 &   0.061& 0.035\nl
     Ca HK &1& \nodata & \nodata &  22.915& 3.117 &  23.927& 1.111 &  19.807& 1.051 &   9.935& 2.564\nl
   CN 4170 &2& \nodata & \nodata &   0.132& 0.040 &   0.054& 0.015 &  -0.003& 0.013 &  -0.082& 0.029\nl
CH = G 4300&1& \nodata & \nodata &   6.687& 1.304 &   4.682& 0.525 &   2.252& 0.540 &   0.393& 1.261\nl
   Fe 4383 &1& \nodata & \nodata &  -1.512& 2.604 &   4.503& 0.836 &   2.203& 0.822 &   0.500& 1.947\nl
   Ca 4455 &1& \nodata & \nodata &   1.372& 1.317 &   1.069& 0.556 &   0.772& 0.494 &  -0.500& 1.208\nl
   Fe 4531 &1& \nodata & \nodata &   3.260& 2.050 &   2.788& 0.802 &   1.788& 0.778 &  -0.534& 1.981\nl
C$_{2}$ 4668 &1& \nodata & \nodata &   4.583& 3.061 &   3.256& 1.163 &   1.289& 1.140 &  -1.491& 2.868\nl
\tablenotetext{1}{1 = Equivalent width (in $\rm \AA$); 2 = magnitude; 3 = 
band ratio or color (in mag)}
\tablenotetext{2}{One-sigma errors.  No errors are calculated for IUE data (M32).}
\end{planotable}

\begin{planotable}{lcrrrrrrrrrrrr}
\tablewidth{0pt}
\tablecaption{Ultraviolet/Violet Spectral Indices and Colors - Elliptical Galaxies}
\tablenum{3b}
\tablehead{
\multicolumn{1}{c}{Feature}        & \multicolumn{1}{c}{Type$^1$} &   \multicolumn{2}{c}{N3605} &
\multicolumn{2}{c}{N3608}               & \multicolumn{2}{c}{N5018} &
\multicolumn{2}{c}{N5831}               & \multicolumn{2}{c}{N6127} &
\multicolumn{2}{c}{N7619}
\\ 
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err$^2$} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err} &
\multicolumn{1}{c}{Obs}		& \multicolumn{1}{c}{Err}
}
\startdata
\hline \nl
 2600--3000 &3&   1.371& 0.032 &   1.018& 0.018 &   1.326& 0.113 &   0.807& 0.021 &   1.266& 0.067 &   0.739& 0.023\nl
Fe II 2402  &2&   0.108& 0.173 &   0.096& 0.087 &  -0.130& 0.949 &   0.057& 0.102 &   0.249& 0.348 &   0.068& 0.111\nl
   BL 2538  &2&   0.475& 0.169 &   0.195& 0.088 &   0.780& 0.771 &   0.189& 0.098 &   0.556& 0.336 &   0.121& 0.102\nl
   Mg Wide  &2&   0.282& 0.027 &   0.235& 0.018 &   0.355& 0.097 &   0.180& 0.022 &   0.230& 0.058 &   0.181& 0.025\nl
Fe II 2609  &2&   0.392& 0.113 &   0.318& 0.063 &   0.165& 0.392 &   0.203& 0.074 &   0.270& 0.223 &   0.142& 0.080\nl
 2609/2660  &3&   0.612& 0.097 &   0.496& 0.056 &   0.473& 0.344 &   0.355& 0.066 &   0.468& 0.200 &   0.298& 0.073\nl
Fe I+II +C  &2&   0.304& 0.099 &   0.184& 0.064 &   0.229& 0.359 &   0.082& 0.079 &   0.248& 0.209 &   0.134& 0.095\nl
Mg II 2800  &2&   0.533& 0.090 &   0.431& 0.060 &   0.611& 0.334 &   0.314& 0.069 &   0.454& 0.185 &   0.173& 0.077\nl
 Mg I 2852  &2&   0.389& 0.072 &   0.448& 0.052 &   0.210& 0.225 &   0.255& 0.060 &   0.484& 0.159 &   0.334& 0.069\nl
 2828/2921  &3&   0.578& 0.062 &   0.552& 0.044 &   0.655& 0.198 &   0.456& 0.053 &   0.475& 0.128 &   0.402& 0.059\nl
 Fe I 3000  &2&   0.252& 0.046 &   0.262& 0.033 &   0.105& 0.133 &   0.207& 0.041 &   0.207& 0.091 &   0.169& 0.047\nl
   BL 3096  &2&   0.172& 0.054 &   0.188& 0.039 &   0.113& 0.150 &   0.135& 0.047 &   0.129& 0.103 &   0.165& 0.054\nl
UV continuum  &3&   1.338& 0.017 &   1.477& 0.012 &   1.236& 0.056 &   1.412& 0.015 &   1.308& 0.032 &   1.481& 0.017\nl
   NH 3360  &1&   4.244& 1.926 &   3.957& 1.409 &  -2.688& 5.696 &   3.040& 1.738 &   2.352& 3.570 &   5.260& 1.886\nl
   Bl 3580  &1&   6.002& 1.841 &  13.540& 1.129 &   9.836& 4.385 &  10.740& 1.509 &   9.823& 2.917 &  11.993& 1.605\nl
    Balmer  &3&   0.697& 0.021 &   0.775& 0.014 &   0.750& 0.054 &   0.833& 0.018 &   0.753& 0.035 &   0.807& 0.019\nl
      4000  &3&   0.716& 0.012 &   0.768& 0.009 &   0.511& 0.029 &   0.769& 0.011 &   0.688& 0.021 &   0.763& 0.012\nl
   CN 3883  &2&   0.314& 0.037 &   0.355& 0.027 &   0.217& 0.087 &   0.347& 0.033 &   0.291& 0.064 &   0.330& 0.036\nl
     Ca HK  &1&  22.533& 2.013 &  24.205& 1.465 &  19.521& 5.211 &  22.761& 1.781 &  24.174& 3.246 &  22.153& 1.845\nl
   CN 4170  &2&   0.068& 0.025 &   0.178& 0.018 &   0.060& 0.065 &   0.150& 0.022 &   0.077& 0.044 &   0.182& 0.025\nl
CH = G 4300  &1&   4.273& 0.936 &   5.060& 0.601 &   3.376& 2.530 &   4.439& 0.772 &   5.696& 1.471 &   5.197& 0.819\nl
   Fe 4383  &1&   5.178& 1.311 &   3.985& 0.940 &   2.136& 3.720 &   4.944& 1.111 &   5.361& 2.343 &   4.325& 1.243\nl
   Ca 4455  &1&   2.357& 0.751 &   1.822& 0.524 &   1.351& 2.177 &   3.340& 0.587 &   2.955& 1.211 &   1.369& 0.727\nl
   Fe 4531  &1&   3.850& 1.247 &   3.320& 0.850 &   3.248& 3.369 &   4.516& 0.979 &   5.492& 0.018 &   3.869& 1.112\nl
C$_{2}$ 4668  &1&   9.645& 1.763 &   7.232& 1.302 &  \nodata&\nodata &   9.313& 1.691 &  \nodata&\nodata 
&  \nodata&\nodata \nl
\tablenotetext{1}{1 = Equivalent width (in $\rm \AA$); 2 = magnitude; 
3 = band ratio or color (in mag)}
\tablenotetext{2}{One-sigma errors.}
\end{planotable}


==> ponder.tab4.tex <==
\begin{planotable}{lccccccc}
\tablewidth{0pt}
\tablecaption{Galactic Globular Cluster Data}
\tablenum{4}
\tablehead{
\multicolumn{1}{c}{NGC Number} &        
\multicolumn{1}{c}{2600--3000$^1$} &
\multicolumn{1}{c}{Mg I 2852$^1$} &
\multicolumn{1}{c}{Mg II 2800$^1$} &
\multicolumn{1}{c}{2609/2660$^1$} &
\multicolumn{1}{c}{2828/2921$^1$} &
\multicolumn{1}{c}{Mg$_2$$^2$} &
\multicolumn{1}{c}{[Fe/H]$^3$}
\\
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{} }

\startdata
\hline\nl
NGC~~104& 1.350& 0.450& 1.060& 0.880& 0.550& \nodata& -0.76 \nl
NGC~~362& 0.740& 0.200& 0.670& 0.530& 0.290& \nodata& -1.16 \nl 
NGC~1904& 0.400& 0.110& 0.450& 0.290& 0.120& \nodata& -1.54 \nl 
NGC~2808& 0.600& 0.150& 0.670& 0.650& 0.310& \nodata& -1.37 \nl 
NGC~5139& 0.500& 0.120& 0.510& 0.370& 0.100& \nodata& -1.62 \nl 
NGC~5272& 0.850& 0.100& 0.700& 0.480& 0.190&  0.042& -1.57 \nl 
NGC~5904& 0.590& 0.210& 0.500& 0.470& 0.280&  0.064& -1.29 \nl 
NGC~6093& 0.390& 0.100& 0.450& 0.290& 0.160& \nodata& -1.62 \nl 
NGC~6205& 0.450& 0.130& 0.440& 0.310& 0.130&  0.043& -1.54 \nl 
NGC~6266& 0.510& 0.220& 0.540& 0.420& 0.240& \nodata& -1.29 \nl 
NGC~6284& 0.400& 0.120& 0.540& 0.280& 0.160& \nodata& -1.32 \nl 
NGC~6293& 0.460& 0.140& 0.350& 0.270& 0.130& \nodata& -1.92 \nl 
NGC~6341& 0.400& 0.110& 0.290& 0.170& 0.100&  0.013& -2.29 \nl 
NGC~6388& 1.100& 0.230& 0.730& 0.820& 0.490& \nodata& -0.60 \nl 
NGC~6441& 1.390& 0.410& 0.830& 1.420& 0.720& \nodata& -0.53 \nl 
NGC~6624& 0.940& 0.450& 0.960& 0.480& 0.600&  0.154& -0.42 \nl 
NGC~6637& 1.150& 0.260& 0.980& 0.820& 0.500&  0.134& -0.71 \nl 
NGC~6681& 0.460& 0.180& 0.490& 0.270& 0.160& \nodata& -1.51 \nl 
NGC~6715& 0.600& 0.200& 0.560& 0.440& 0.170& \nodata& -1.59 \nl 
NGC~6752& 0.420& 0.110& 0.550& 0.330& 0.200& \nodata& -1.55 \nl 
NGC~6864& 0.890& 0.290& 0.620& 0.580& 0.110& \nodata& -1.32 \nl 
NGC~7078& 0.470& 0.120& 0.330& 0.230& 0.120&  0.017& -2.22 \nl 
NGC~7089& 0.450& 0.160& 0.490& 0.320& 0.120&  0.052& -1.62 \nl 
NGC~7099& 0.310& 0.090& 0.320& 0.200& 0.020& \nodata& -2.12 \nl
\tablenotetext{1}{Line strengths and spectral breaks from Rose \& Deng (1998),
as measured from IUE LWP data. No poisson errors are calculable for the IUE
data.}
\tablenotetext{2}{Optical Mg$_2$ taken from BFGK (1984).}
\tablenotetext{3}{[Fe/H] values taken from WEB page of Harris (1997)}

\end{planotable}


==> ponder.tab5.tex <==
\begin{planotable}{rccl}
\tablewidth{0pt}
\tablecaption{2600-3000 Colors for Davidge and Clark Stars} 
\tablenum{5a}
\tablehead{
\\
\multicolumn{1}{c}{HD} &        
\multicolumn{1}{c}{2600--3000} &
\multicolumn{1}{c}{Src$^1$} &
\multicolumn{1}{c}{Sp Typ$^2$} 
\\
\multicolumn{1}{c}{} &        
\multicolumn{1}{c}{mag} &        
\multicolumn{1}{c}{} &        
\multicolumn{1}{c}{}  
}

\startdata
\hline \nl
 72324 & 2.58 &1& G9~III  \nl
 75732 & 2.31 &1& G8~V    \nl
 90277 & 0.73 &2& F0~V    \nl
102634 & 1.35 &2& F7~V    \nl
111631 & 2.90 &2& M0.5~V  \nl
114710 & 1.56 &1& G0~V    \nl
139669 & 2.35 &2& K5~III  \nl
146051 & 1.73 &2& M0~III  \nl
148856 & 2.39 &2& G7~III  \nl
149661 & 2.01 &2& K2~V    \nl
154633 & 1.82 &2& G5~V    \nl
154733 & 2.35 &2& K4~III  \nl
156653 & 0.08 &2& A1~V    \nl
187642 & 0.40 &2& A7~V    \nl
\tablenotetext{1}{Source of 2600--3000 color: 1 = from Fanelli et al. (1990)
direct observation; 2 = inferred from stellar groups as determined by
Fanelli et al. (1992).}
\tablenotetext{2}{Spectral Types as listed by Davidge \& Clark (1994).}

\end{planotable}

\begin{planotable}{rlcrcrlcr}
\tablewidth{0pt}
\tablecaption{Lick CN4170, 2600--3000 Measures for Stars} 
\tablenum{5b}
\tablehead{
\\
\multicolumn{1}{c}{HD Number} &        
\multicolumn{1}{c}{Sp Typ$^1$} &
\multicolumn{1}{c}{2600--3000$^2$} &
\multicolumn{1}{c}{CN4170$^3$} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{HD Number} &        
\multicolumn{1}{c}{Sp Typ$^1$} &
\multicolumn{1}{c}{2600--3000$^2$} &
\multicolumn{1}{c}{CN4170$^3$} 
\\
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} 
}

\startdata
\hline \nl

   1461 &  G0~V  & 2.00 & -0.018&$\vert$&  4307 & G0~V   &1.66 & -0.071 \nl
   4614 &  GO~V  & 1.31 & -0.073&$\vert$&  6203 & K0~III &3.00 &  0.150 \nl 
  10307 &  G2~V  & 1.56 & -0.061&$\vert$& 10380 & K3~III &2.98 &  0.208 \nl 
  10476 &  K1~V  & 2.12 & -0.018&$\vert$& 10700 & G8~V   &1.74 & -0.059 \nl
  10780 &  K0~V  & 2.15 & -0.050&$\vert$& 13043 & G2~V   &1.84 & -0.073 \nl
  14802 &  G1~V  & 1.76 & -0.072&$\vert$& 17709 & K7~III &1.40 &  0.114 \nl
  19476 &  K0~III& 2.67 &  0.217&$\vert$& 20630 & G5~V   &1.88 & -0.034 \nl
  22879 &  F9~V  & 1.13 & -0.069&$\vert$& 30455 & G2~V   &1.58 & -0.075 \nl
  35620 &  K3~III& 2.92 &  0.358&$\vert$& 37160 & K0~III &2.73 &  0.027 \nl
  48682 &  G0~V  & 1.72 & -0.053&$\vert$& 49293 & K0~III &2.68 &  0.287 \nl
  51440 &  K2~III& 3.14 &  0.120&$\vert$& 54719 & K2~III &2.90 &  0.324 \nl
  55575 &  G0~V  & 1.56 & -0.107&$\vert$& 64606 & G8~V   &1.74 & -0.075 \nl
  66141 &  K2~III& 3.07 &  0.140&$\vert$& 67767 & G7~V   &2.11 &  0.035 \nl
  69267 &  K4~III& 2.35 &  0.202&$\vert$& 70272 & K4.5~I &2.47 &  0.165 \nl
  72184 &  K2~III& 2.95 &  0.275&$\vert$& 72324 & G9~III &2.57 &  0.259 \nl
  73471 &  K2~III& 3.14 &  0.337&$\vert$& 75732 & G8~V   &2.30 &  0.112 \nl
  82328 &  F6~IV & 1.16 & -0.116&$\vert$& 85503 & K2~III &2.79 &  0.388 \nl
  90508 &  F9~V  & 1.63 & -0.079&$\vert$& 95272 & KO~III &3.04 &  0.286 \nl
 101501 &  G8~V  & 1.98 & -0.007&$\vert$&102870 & F8~V   &1.56 & -0.040 \nl
 114710 &  G0~V  & 1.56 & -0.070&$\vert$&115043 & G1~V   &1.63 & -0.074 \nl
 115617 &  G6~V  & 1.91 & -0.054&$\vert$&117176 & G2.5~V &2.08 & -0.044 \nl
 121370 &  G0~IV & 1.44 & -0.072&$\vert$&125560 & K3~III &2.98 &  0.294 \nl
 132345 &  K3~III& 2.91 &  0.459&$\vert$&134083 & F5~V   &1.20 & -0.119 \nl
 137759 &  K2~III& 2.85 &  0.247&$\vert$&140573 & K2~III &3.01 &  0.352 \nl
 142373 &  F8~V  & 1.42 & -0.087&$\vert$&142860 & F6~V   &1.34 & -0.117 \nl
 145328 &  K0~III& 2.74 &  0.138&$\vert$&145675 & K0~V   &2.31 &  0.088 \nl
 152792 &  G0~V  & 1.68 & -0.036&$\vert$&161797 & G5~IV  &2.00 &  0.009 \nl
 163506 &  F2~IA & 1.16 & -0.065&$\vert$&182572 & G8~IV  &2.15 &  0.011 \nl
 185144 &  K0~V  & 1.96 & -0.031&$\vert$&187691 & F8~V   &1.69 & -0.080 \nl
 187923 &  G0~V  & 1.83 & -0.030&$\vert$&188512 & G8~IV  &2.21 &  0.006 \nl
 197076 &  G5~V  & 1.80 & -0.095&$\vert$&198149 & K0~IV  &2.37 &  0.079 \nl
 199629 &  A0~V  & 0.01 & -0.063&$\vert$&200580 & F9~V   &1.21 & -0.063 \nl
 207978 &  F6~IV-& 0.94 & -0.116&$\vert$&209750 & G2~IB  &1.81 & -0.078 \nl
 210027 &  F5~V  & 1.15 & -0.078&$\vert$&211038 & G8~V   &2.55 &  0.043 \nl
 215648 &  F6~III& 1.34 & -0.083&$\vert$&216385 & F7~IV  &1.31 & -0.126 \nl
 217877 &  F8~V  & 1.69 & -0.091&$\vert$&219134 & K3~V   &2.31 &  0.062 \nl
 222368 &  F7~V  & 1.45 & -0.080&$\vert$&224930 & G2~V   &1.52 & -0.085 \nl
\tablenotetext{1}{Spectral Types as listed by Fanelli et al. (1990)}
\tablenotetext{2}{IUE 2600--3000 colors taken from Li et al. (1998).}
\tablenotetext{3}{CN4170 on original Lick system, from Worthey et al. (1994).}
\end{planotable}

\begin{planotable}{lccc}
\tablewidth{0pt}
\tablecaption{Elliptical Galaxy Mg$_2$, IUE 2600-3000 Colors} 
\tablenum{5c}
\tablehead{
\\
\multicolumn{1}{c}{NGC Number} &        
\multicolumn{1}{c}{Mg$_2$$^1$} &
\multicolumn{1}{c}{2600--3000$^2$} &
\multicolumn{1}{c}{} 
\\
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{mag} &
\multicolumn{1}{c}{} }

\startdata
\hline \nl

M~31  & 0.332 & 1.199 & \nl
N~4382& 0.234 & 1.189 & \nl
N~4472& 0.342 & 1.353 & \nl
N~4552& 0.351 & 0.839 & \nl
N~4621& 0.351 & 1.150 & \nl
N~4649& 0.373 & 0.835 & \nl
N~5102& 0.046 & 0.345 & \nl
\tablenotetext{1}{Mg$_2$ measures taken from Trager et al. (1998).}
\tablenotetext{2}{IUE 2600--3000 colors taken from Burstein et al. (1988).}
\end{planotable}

